Understanding Information Disclosure from Secure Computation Output: A Study of Average Salary Computation

Secure multi-party computation has seen substantial performance improvements in recent years and is being increasingly used in commercial products. While a significant amount of work was dedicated to improving its efficiency under standard security models, the threat models do not account for information leakage from the output of secure function evaluation. Quantifying information disclosure about private inputs from observing the function outcome is the subject of this work. Motivated by the City of Boston gender pay gap studies, in this work we focus on the computation of the average of salaries and quantify information disclosure about private inputs of one or more participants (the target) to an adversary via information-theoretic techniques. We study a number of distributions including log-normal, which is typically used for modeling salaries. We consequently evaluate information disclosure after repeated evaluation of the average function on overlapping inputs, as was done in the Boston gender pay study that ran multiple times, and provide recommendations for using the sum and average functions in secure computation applications. Our goal is to develop mechanisms that lower information disclosure about participants' inputs to a desired level and provide guidelines for setting up real-world secure evaluation of this function.

==> commands.tex <==

\let\oldtextbf\textbf
\renewcommand{\textbf}[1]{\oldtextbf{\boldmath #1}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}


\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{claim}{Claim}[]


\newcommand{\eq}{\Leftrightarrow}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


\renewcommand{\vec}[1]{\mathbf{#1}}


\newcommand{\norm}[1]{\left\lvert#1\right\rvert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\renewcommand{\Pr}[1]{\text{Pr}\left[#1\right]}
\newcommand{\lp}[1]{\left(#1\right)}
\newcommand{\lb}[1]{\left[#1\right]}
\newcommand{\lbr}[1]{\left\{#1\right\}}
\newcommand{\lng}[1]{\left\langle#1\right\rangle}

\newcommand{\Ex}[1]{\text{E}\left[#1\right]}
\newcommand{\Cov}[1]{\text{Cov}\left[#1\right]}
\newcommand{\Var}[1]{\text{Var}\left[#1\right]}


\newcommand{\tran}{\text{T}}


\newcommand{\summ}[2]{\sum_{#1}^{#2}}
\newcommand{\intt}[2]{\int_{#1}^{#2}}
\newcommand{\prodd}[2]{\prod_{#1}^{#2}}


\newcommand*{\qedb}{\null\nobreak\hfill\ensuremath{\blacksquare}}%
\newcommand{\xor}{\oplus}


\newcommand{\negl}{\textsf{negl}}

\newcommand{\nin}{\notin}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\T}{\mathcal{T}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\grp}{\mathcal{G}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\NP}{\mathcal{NP}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\of}{\subseteq}
\newcommand{\fo}{\supseteq}
\newcommand{\nof}{\subsetneq}
\newcommand{\nfo}{\supsetneq}
\newcommand{\emp}{\emptyset}
\newcommand{\val}{\text{val}}
\newcommand{\spn}{\text{span}}
\newcommand{\rank}{\text{rank}}
\newcommand{\argmax}{\text{argmax}}

\newcounter{casenum}
\newenvironment{caseof}{\setcounter{casenum}{1}}{\vskip.5\baselineskip}
\newcommand{\case}[2]{\vskip.5\baselineskip\par\noindent {\bfseries Case \arabic{casenum}:} #1\\#2\addtocounter{casenum}{1}}



\newcommand{\Mod}{\ \mathrm{mod}\ }


\renewcommand{\And}{\textbf{and} }

==> conclusion.tex <==

\section{Conclusion} % (fold)
\label{sec:Conclusion}



==> experiments.tex <==




\subsection{Single Calculation} % (fold)
\label{sub:Single Calculation}
The simplest configuration we consider is a single computation of an average
$O = X_T + X_S$.

\subsubsection{Poisson} % (fold)
\label{ssub:Poisson}
Suppose all participants inputs' are modeled by the Poisson distribution. We assume the parameter $\lambda$ is the same for random variables to simplify our analysis and experiments, but this is not required. 

\begin{figure}[t]
    \begin{small}
        \begin{center}
            \includegraphics[width=0.85\textwidth]{multiple_dists.pdf}
        \end{center}
        \caption{Entropy measure as the number of spectators increase in a single computation.}
        \label{fig:multiple_dists}
    \end{small}
\end{figure}

\begin{figure}[t]
    \begin{small}
        \begin{center}
            \includegraphics[width=0.85\textwidth]{entropy_loss}
        \end{center}
        \caption{Relative entropy loss as the number of spectators increase in a single computation.}
        \label{fig:entropy_loss}
    \end{small}
\end{figure}


\subsection{Two Calculations} % (fold)
\label{sub:Two Calculations}

\subsubsection{Shared Spectator Presence} % (fold)
\label{ssub:Shared Spectator Presence}

\begin{figure}[t]
    \begin{small}
        \begin{center}
            \includegraphics[width=0.85\textwidth]{0_vs_1_shared_spec}
        \end{center}
        \caption{Impact of the presence of a shared spectator on target information loss.}
        \label{fig:0_vs_1_shared_spec}
    \end{small}
\end{figure}




\subsubsection{Participating Once vs. Twice} % (fold)
\label{ssub:Participating Once vs. Twice}

\begin{figure}[t]
    \begin{small}
        \begin{center}
            \includegraphics[width=0.85\textwidth]{out_1_vs_2_2048}
        \end{center}
        \caption{Target information loss after participating in one or two computations. Not shown: if the target participates in one experiment and all the shared spectators are reused, then $h(X_T \mid O_1, O_2') =0$.}
        \label{fig:out_1_vs_2_2048}
    \end{small}
\end{figure}



==> misc.tex <==


\section{Entropy}
Some useful properties of entropy and conditional entropy:

For any two random variables:
\begin{align}
	H(X,Y)&=H(X)+H(Y|X)=H(Y)+H(X|Y);\\
	H(X,Y)&=H(X)+H(Y) \text{ if $X$ and $Y$ are independent.}\\
	H(X+Y|X)&=H(Y|X);\\
	H(Y|X)&=H(Y) \text{ if $X$ and $Y$ are independent.}\\
	H(Y|X)&= -\sum_{x \in \X }^{ } \sum_{y \in \Y }^{} p(x,y) \log p(y \mid x)\\
	&= -\sum_{x \in \X }^{ } \sum_{y \in \Y }^{} p(x,y) \log {\frac{p(x,y)}{p(x)}}\\
	H(X,Y)&= -\sum_{x \in \X }^{ } \sum_{y \in \Y }^{} p(x,y) \log p(x,y)
\end{align}

\section{Characteristic Function}

Consider a random variable $X$. Define its characteristic function:
\begin{align}
	\Phi_X(\omega)=\me[e^{i\omega X}],
\end{align}
where $i$ is the imaginary unit. The inversion can be computed by inverse Fourier transform. 
One nice property we would like to employ is that if we consider the sum of two independent random variables: $Z=X +Y$, 
then the  characteristic function of $Z$ is the multiplication of characteristic functions of $X$ and $Y$, which can be computed:
\begin{align}
	\Phi_Z(\omega)=\Phi_X(\omega)\Phi_Y(\omega).
\end{align}
 Then an inversion can be done on the characteristic function of $Z$ to obtain the probability distribution function of $Z$.




\section{Derivation of Poisson PMF} % (fold)
\label{sec:derivation_of_poisson_pmf}


The characteristic function of a Poisson random variable is (for $\lambda \in \R_{> 0}$)
\begin{align*}
\Phi_X(t)  &= e^{\lambda \lp{e^{it} - 1} } \\
&= e^{- \lambda} \lp{\summ{ k = 0}{ \infty} \frac{\lambda^k e^{i t k}}{k!}},
\end{align*}
where we use the Taylor Series  of $e^x$ with $x = \lambda e^{it}$. We use the following inversion formula to recover the pmf from the characteristic function:
\begin{align*}
p_{X}(a) = \Pr{X = a} = \lim_{T \to \infty} \frac{1}{2T} \int_{-T}^{T} e^{-i t a} \Phi_{X} \lp{t} dt.
\end{align*}
Computing the integral:
\begin{align*}
\int_{-T}^{T} e^{-i t a} \Phi_{X} \lp{t} dt &= \int_{-T}^{T} e^{-i t a}  e^{- \lambda} \lp{\summ{ k = 0}{ \infty} \frac{\lambda^k e^{i t k}}{k!}} dt  
= e^{\lambda} \summ{ k = 0}{ \infty}  \frac{\lambda^k }{k!}\int_{-T}^{T} e^{i t (k - a)} dt.
\end{align*}
The above integral can be split into two cases:
\begin{enumerate}[label=\emph{(Case \arabic*)},leftmargin=3\parindent]
	\item If $k = a$, then
\begin{align*}
\int_{-T}^{T} e^{-i t (k - a)} dt = 2T.
\end{align*}
\item If $k \neq a$, then 
\begin{align*}
\int_{-T}^{T} e^{-i t (k - a)} dt = \int_{-T}^{T} \cos \lb{(k - a) t}dt  = \frac{2}{k - a} \sin \lb{(k-a) T}.
\end{align*}
\end{enumerate}
Therefore, the integral evaluates to 
\begin{align*}
2T e^{-\lambda} \frac{\lambda^a}{a!} + 2 e^{-\lambda} \summ{ k \neq a}{ }\frac{\lambda^k \sin \lb{(k-a) T}}{k!(k - a)} .
\end{align*}
Lastly, we compute the limit and use the dominated convergence theorem to swap the limit and summation:
\begin{align*}
\lim_{T \to \infty} \frac{1}{2T} \left\{ 2T e^{-\lambda} \frac{\lambda^a}{a!} \right. +\left. 2 e^{-\lambda} \summ{ k \neq a}{ }\frac{\lambda^k \sin \lb{(k-a) T}}{k!(k - a)} \right\} 
 &=  e^{-\lambda} \frac{\lambda^a}{a!}  + 2 e^{-\lambda} \lim_{T \to \infty} \frac{1}{2T} \lp{ \summ{ k \neq a}{ }\frac{ \lambda^k\sin \lb{(k-a) T}}{k!(k - a)} } \\
 &=  e^{-\lambda} \frac{\lambda^a}{a!}  + 2 e^{-\lambda} \summ{ k \neq a}{ } \underbrace{ \lim_{T \to \infty} \frac{\lambda^k \sin \lb{(k-a) T}}{2 k!(k - a) T} }_{= 0} \\
 &=  e^{-\lambda} \frac{\lambda^a}{a!}.
\end{align*}

Now, suppose we have a sum of $n$ Poisson random variables, such that
\begin{align*}
X_{S} = \sum_{j=1}^nX_{S_j}.
\end{align*}
The characteristic function of $X_S$ becomes (from the property above)
\begin{align*}
\Phi_{X_{S}} = \prod_{j = 1}^{n} \Phi_{X_{S_j}} &= e^{\lambda \lp{e^{it} - 1} }   e^{\lambda \lp{e^{it} - 1} }  \dots   e^{\lambda \lp{e^{it} - 1} } 
= e^{\lambda n \lp{e^{it} - 1} }
= e^{- \lambda n} \lp{\summ{ k = 0}{ \infty} \frac{\lp{ \lambda n}^k e^{i t k}}{k!}}.
\end{align*}
Interestingly, this only slightly changes the final result from above, where $e^{- \lambda}$ becomes $e^{- \lambda n}$ and $\lambda^k $ becomes $(\lambda n)^{k}$. Therefore, the pmf of the sum of $n$ Poisson random variables is 
\begin{align*}
p_{X_s}(a) = \Pr{X_s = a} =  e^{-\lambda n} \frac{(\lambda n )^a}{a!}.
\end{align*}
For the sake of computability, we add an alternate formulation that leverages the gamma function $\Gamma (n) = (n-1)!$
\begin{align*}
p_{X_s}(a) = \Pr{X_s = a} = \exp \lb{a \ln \lambda n - \lambda n - \ln \Gamma(a + 1)}.
\end{align*}







==> packages.tex <==

\usepackage[in]{fullpage}
\usepackage[dvipsnames]{xcolor}

\usepackage[
bookmarksopen,
bookmarksdepth=2,
colorlinks=false,
hidelinks
]{hyperref}

\usepackage{authblk}
\usepackage{blindtext}
\usepackage{wrapfig}
\setlength{\parskip}{.5em}
\usepackage{svg}

\usepackage{changepage}



\usepackage{authblk}
\usepackage{xfrac}


\usepackage{appendix}
\usepackage{soul}

\usepackage{inconsolata}
\usepackage{graphicx}% Include figure files
\usepackage{subcaption}% Include figure files

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}


\usepackage{bm}% bold m
\usepackage{float}
\usepackage{tabularx}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{tikz}
\usepackage{enumerate}
\usepackage{multirow}
\usepackage{mathtools}

\usepackage{silence}
  \WarningFilter*{latex}{Label `' multiply defined}
  \WarningFilter*{latex}{There were multiply-defined labels.}
\WarningsOff

\usepackage{mathtools}
\usepackage{listings}

\usepackage[inline]{enumitem}
\setlist{nosep} % or \setlist{noitemsep} to leave space around whole list


